Generative Language-Grounded Policy in Vision-and-Language Navigation with Bayes' Rule

Vision-and-language navigation (VLN) is a task in which an agent is embodied in a realistic 3D environment and follows an instruction to reach the goal node. While most of the previous studies have built and investigated a discriminative approach, we notice that there are in fact two possible approaches to building such a VLN agent: discriminative \textit{and} generative. In this paper, we design and investigate a generative language-grounded policy which uses a language model to compute the distribution over all possible instructions i.e. all possible sequences of vocabulary tokens given action and the transition history. In experiments, we show that the proposed generative approach outperforms the discriminative approach in the Room-2-Room (R2R) and Room-4-Room (R4R) datasets, especially in the unseen environments. We further show that the combination of the generative and discriminative policies achieves close to the state-of-the art results in the R2R dataset, demonstrating that the generative and discriminative policies capture the different aspects of VLN.

==> vln.tex <==
\section{Background: Vision-and-Language Navigation}



%Vision-and-Language navigation is a task that an agent follows an given instruction, explore in the realistic 3D modeling and reach the destination place specified by the instruction.

% As is shown in Fig, XX

In the R2R dataset~\citep{mattersim}, an agent moves on a graph that was constructed from one of the realistic 3D models of houses and buildings based on Matteport 3D dataset~\citep{Matterport3D}.
At the beginning of each trial, the agent is given textual instruction, is placed at the start node and attempts to reach at the goal node by moving along the edges.
At each node of the graph the agent observes the visual features of the surrounding environment and makes a decision to which neighbour node it will move next.
When the agent determines that the current node is sufficiently close to the destination node, it outputs ``STOP'', and the navigation trial ends.
The agent is evaluated in terms of the accuracy of their final location and the trajectory length \citep{mattersim,spl}.

The difficulties in VLN mainly arise from the diversity of textual instructions.
R2R provides multiple instructions for each trajectory. These instructions are created via crowd-sourcing, and their granularity and specificity highly vary \citep{vln-press}.
The agent futhermore needs to generalize to unseen environments.
Previous studies have reported that models with rich visual and textual features often overfit to the seen environments~\citep{vln-areyoulooking}.

%is an essential task that allow an virtual agent to understand instruction text given by humans and try to follow it \cite{mattersim}. The virtual agent is embodied in realistic 3D environment and it can move on a graph that is embodied in 3D modelings that are scanned from real houses and buildings. At the first, the agent is placed in the initial point of the 3D model and then given one of textual instructions that indicate the route to the goal place. Instructions are created via crowd-sourcing and hence have ambiguities.  The agent need to follow the instructions, observe the surrounding visual features and take actions to find out the goal place.

%VLN is a natural task for Human because we often visit unfamiliar places and search for the objective place with navigation of others. Human score of VLN is quite high...

%The difficulties of VLN is that the textual instructions are robust and varies.

%The R2R navigation dataset includes there or four annotated instructions per trajectory.
%\citep{vln-press} proposed a model that takes as inputs multiple instructions to predict a single trajectory. Combined with pretrained language models, their model with multiple instructions achieve much greater results than models with single instructions.
%as of Table.2 in their paper.
%However multiple instructions are not always available in realistic navigation problem.% in because we decide not to allow our models to make use of multiple instructions because they are not always available in realistic navigation settings.

%For humans, given a robust and fazzy instruction, they can make some plans to follow the instructions. In this paper we proposed language-grounded policy to allow models to build a predictions based on language models that contributes the global planning.
%In some cases, they choose a decision that would possibly reconstruct the whole instruction later.


%Humans have with no-doubts higher abilities to recognize the surrounding situations, remember the past occurrences and make some concrete plans for their final objections. After creating concrete plans with languages, humans make some decisions what to do the next so that the decided actions will maximize the possibility to reach the final objections. Especially, humans use languages not only for communicating with others but also for thinking, planing and the decision making in their interior.


%to navigate a virtual agent interior of
%(We might need a Figure for VLN task here.)
